Learning drivers of climate-induced human migrations with Gaussian processes

In the current context of climate change, extreme heatwaves, droughts, and floods are not only impacting the biosphere and atmosphere but the anthroposphere too. Human populations are forcibly displaced, which are now referred to as climate-induced migrants. In this work, we investigate which climate and structural factors forced major human displacements in the presence of floods and storms during the years 2017-2019. We built, curated, and harmonized a database of meteorological and remote sensing indicators along with structural factors of 27 developing countries worldwide. We show how we can use Gaussian Processes to learn what variables can explain the impact of floods and storms in the context of forced displacements and to develop models that reproduce migration flows. Our results at regional, global, and disaster-specific scales show the importance of structural factors in the determination of the magnitude of displacements. The study may have both societal, political, and economical implications.

==> supertable.tex <==

\begin{footnotesize}
\begin{tabular}{p{3cm}p{3cm}p{3cm}p{3cm}p{3cm}}
\toprule \toprule
{\bf Feature} & {\bf Short} & {\bf Years} & {\bf Description} & {\bf Reference} \\\midrule
\multicolumn{5}{l}{{\bf Domain: \textit{Migration}}}\\ 
\midrule
Internally Displaced Person & IDP & 2017-2019 & Person forced to leave home, in particular as a response of a climate disaster and that has not crossed any international border. & IDMC web \cite{IDMCweb} \\
\midrule
\multicolumn{5}{l}{{\bf Domain: \textit{Atmospheric}}}\\ 
\midrule
Evapotranspiration & Eva & 2017-2019 & Evapotranspiration maxima from VIC4.1.2 (and Noah3.3) is the sum of three weighted components by their surface contribution: canopy intercepted evaporation, vegetation transpiration and earth evaporation. Units: kg m-2 s-1. & FLDAS Noah Land Surface Model L4 Global Monthly 0.1 x 0.1 degree \cite{FDLAS1} \\
\midrule

Specific Humidity & Hum    & 2017-2019 & Units: kg kg-1 & FLDAS Noah Land Surface Model L4 Global Monthly 0.1 x 0.1 degree \cite{FDLAS1} \\
\midrule

Total Precipitation Rate            & PrR & 2017-2019 & Monthly total precipitation rate combining data from GDAS, MERRA-2 and CHIRPS. Units: kg m-2 s-1                                 & FLDAS Noah Land Surface Model L4 Global Monthly 0.1 x 0.1 degree \cite{FDLAS1}                      \\ \midrule

Wind Speed 1               & Ws1    & 2017-2019 & Wind speed at surface level (10m). Units: m s-1                                                                                                                           & FLDAS Noah Land Surface Model L4 Global Monthly 0.1 x 0.1 degree \cite{FDLAS1}                                                                                                            \\ \midrule

Near Surface Temperature (2m) & T      & 2017-2019 &  Units: K                                                                                   & FLDAS Noah Land Surface Model L4 Global Monthly 0.1 x 0.1 degree \cite{FDLAS1}.                                                                                            \\ \midrule                                                                                                         
Water Vapour Pressure                    & Vap    & 2017-2019 & Measure of the vertical column of water vapour Measure combining meteorological station datas of  WorldClim v2, CRU Ts4.0 and JRA-55 Units: kPa                                                                                                                                                                                                                                                                   & TerraClimate: Monthly Climate and Climatic Water Balance for Global Terrestrial Surfaces 2.5 arc minutes \cite{terra}                                                                                                                                                                                            \\ \midrule
Water Vapour Deficit                 & Vpd & 2017-2019 & Measure of monthly water deficit around mean value of the dataset combining meteorological station datas of  WorldClim v2, CRU Ts4.0 and JRA-55 Units: kPa                                                            & TerraClimate: Monthly Climate and Climatic Water Balance for Global Terrestrial Surfaces 2.5 arc minutes \cite{terra}                                                                                                                                                                                              \\ \midrule

Precipitation Accumulation                & PrA    & 2017-2019 & Measure of monthly accumulated precipitation combining meteorological station datas of  WorldClim v2, CRU Ts4.0 and JRA-55 Units: mm                                                                                                                                                                                                                                 & TerraClimate: Monthly Climate and Climatic Water Balance for Global Terrestrial Surfaces 2.5 arc minutes \cite{terra}                                                                                                                                                                                              \\ \midrule


Mean Total Precipitation               & TPr  & 2017-2019 & Precipitation rate over earth surface if it was uniformly distributed over the selected region. Precipitation is generated following ECMWF "Integrated Forecasting System" (IFS) models. Units: kg m-2 s-1                                                                                                            & ERA5 Monthly aggregates 0.25 arc degrees -  ECMWF / Copernicus Climate Change Service \cite{era5}                                                                                                                                                                                                                 \\ \midrule

Wind Speed 2                       & Ws2    & 2017-2019 & Horizontal wind component at 10m. Unidades: m s-1                                                                                                                                                                                                                                    & ERA5 Monthly aggregates 0.25 arc degrees -  ECMWF / Copernicus Climate Change Service \cite{era5}                                                                                                                                                                                                              \\ \midrule

Sea Level Pressure                           & Pres    & 2017-2019 & Minima of atmospheric pressure adjusted to sea level altitude. Se utiliza para identificar centros de baja y alta presión. Unidades: Pa.                                                                                                                                                                                                                                                                                                        & ERA5 Monthly aggregates 0.25 arc degrees -  ECMWF / Copernicus Climate Change Service \cite{era5}     
       \\ \midrule
\multicolumn{5}{l}{{\bf Domain: \textit{Earth}}}\\ 
\midrule
       
Soil Moisture                         & Soil   & 2017-2019 & Soil moisture at 0 - 10 cm underground. Units: m\textasciicircum{}3 m-3                                                                                                                                                                        & FLDAS Noah Land Surface Model L4 Global Monthly 0.1 x 0.1 degree \cite{FDLAS1}                                                                                                                                                                                                             \\ \midrule
Water Run-off                 & Run    & 2017-2019 & In Noah3.3, water Run-off is computed using the two layers conceptual scheeme of Schaake et al.37 based on a simple water balance model. Units: kg m-2 s-1 & FLDAS Noah Land Surface Model L4 Global Monthly 0.1 x 0.1 degree \cite{FDLAS1}                                                                                                                                                                                                             \\ \midrule
Underground Water Run-off          & Urun   & 2017-2019 & Units: kg m-2 s-1                                                                                                                                                                                                                                                                                                                                                                                                                                                                   & FLDAS Noah Land Surface Model L4 Global Monthly 0.1 x 0.1 degree \cite{FLDAS1}                                                                                                                                                                                                             \\ \midrule
\multicolumn{5}{l}{{\bf Domain: \textit{Demographic}}}\\ 
\midrule
Total Population                & Pop    & 2015    & Population density estimate based on national registers adjusted by the "United Nation's World Population Prospects" (UN WPP) census in 2015 multiplied by the area of the affected region  & GPWv411: Population Density (Gridded Population of the World Version 4.11) \cite{pop} \\ \midrule


Rural Population                     & RP     & 2018         & percentage of Rural Population the country.                                                                                                                                                                                                                                                                                                                                                                               &     United Nations Development Programme: Human Development Reports \cite{UN}                                                                                                                                                                                                                                                                                                      \\ \midrule
Birth Rate                  & BR     & 2018         &   Birth Rate in the country.                                                                                                                                                          &United Nations Development Programme: Human Development Reports \cite{UN}                                                                                                                                                                                                                                                                                                           \\ \midrule
Life Expectancy                      & LE     & 2018         &    Average Life Expectancy in the country.                                                                                                                                                                                                                                                                                         & United Nations Development Programme: Human Development Reports \cite{UN}                                                                                                                                                                                                                                                                                               \\ \midrule
Median Age                           & MA     & 2018         & Median Age of the population of the country                                                                                                                                                                                                                                                                                  &  United Nations Development Programme: Human Development Reports \cite{UN}                                                                                                                                                                                                                                                                                                      \\ \midrule
Unemployment                                 & UN     & 2018         & Unemployment percentage in the country.                                                                                                                                                                                                                                                                                   &  United Nations Development Programme: Human Development Reports \cite{UN}                                                                                                                                                                                                                                                                                                         \\ \midrule
\multicolumn{5}{l}{{\bf Domain: \textit{Socio-economic variable}}}\\ 
\midrule
Mortality due to lack of sanitation          & MS     & 2018         & Number of deaths due to poor hygiene and sanitary services per 100.000 inhabitants in the country.                                                                                                                                                                                                                                                                                                                                                                                                                                                             &           United Nations Development Programme: Human Development Reports \cite{UN}                                                                                                                                                                                                                                                                                                \\ \midrule
GDP per Capita                        & GDP    & 2018         & FMI establishes establece dat ``GDP measures the monatary value of final goods and services, that are bought by the final user, produced in a country per capita''                                                                                                                                                                                                                                                                                               &    World Development Indicator \cite{WDI}                                                                                                                                                                                                                                                                                                        \\ \midrule
Exports \& Imports                    & EI     & 2018         &    It's a measurement on the trade of a country. measures the total exports and imports in dollars as a \% of the GDP of the country.                                                                                                                                                                                               &       United Nations Development Programme: Human Development Reports \cite{UN}                                                                                                                                                                                                                                                                                                    \\ \midrule
Electricity Access                & AE     & 2018         &   Percentage of the population with access to electricity                                                                                                                                                                                                      &    United Nations Development Programme: Human Development Reports \cite{UN}                                                                                                                                                                                                                                                                                                       \\ \midrule
Cereal Yield                        & CY     & 2018         &    Kg of cereals produced in the country.                                                                                                                                                                                                          &                 United Nations Development Programme: Human Development Reports \cite{UN}                                                                                                                                                                                                                                                                                          \\ \midrule
Employment in Agriculture                               & EA     & 2018         &  Fracction of total employment that belong to agricultural practises.                                                                                                                                                                                                                                                                                                 &                       United Nations Development Programme: Human Development Reports \cite{UN}                                                                                                                                                                                                                                                                                    \\ \midrule
Paved Road                            & PR     & 2018         & km of paved road in the country.                                                                                                                                                                                                                     &      United Nations Development Programme: Human Development Reports \cite{UN}                                                                                                                 \\ \midrule
\multicolumn{5}{l}{{\bf Domain: \textit{Socio-economic Index}}}\\ 
\midrule
Human Inequality                              & HI     & 2018         &     Measures the capability of citizens of accessing the same life conditions in a country if inequality conditions did not exist. &  World Development Indicator \cite{WB}                                                                                                                                                      \\ \midrule
Concentration Index                              & CI     & 2018         &  Defined as twice the area below the concentration curve, $L(p)$, and the line of equality. In case of not existing salary equality CI is equal to 0.                                                                                                                                                  & World Development Indicator \cite{WB}                                                                                                                                                                                          \\ \midrule
Education Index                       & EDI    & 2018         &  50\% weighted average between the mean years of adult scholarization and the mean years of children scholarization.                                                                                                                                                                                                                                                                       & World Development Indicator \cite{WB}                                                                                                                                                                                                \\ \midrule
Human Development Index               & HDI    & 2018         &  Summarizes a measurement of the development in the country: A health, life expectancy, education and life quality.HDI is the geometric average between life expectancy, Education Index and Income Index.                                                                                                                                                                               &  World Development Indicator \cite{WB}                                                                                                                   \\ \midrule
Income Index                          & II     & 2018         & Income Index o GNI per capita is defined as the GDP plus foreign money influx minus the money leaving the country per capita.                                                                &         World Development Indicator \cite{WB}                                                                                                                                                                                             \\ \midrule
Human Capital Index                   & HCI    & 2018         &            The index measures the capability of the country to mobilize the economic and profesional potential of its citizens. It also measures the capital loses trough a lack of education and sanitation.                                                                                                                                                                   &      World Development Indicator \cite{WB}                                                                                                        \\ \midrule
\multicolumn{5}{l}{Domain: \textit{Environmental}}\\ 
\midrule
Coastline                            & CO     & Static       &     Km of coastline in the area.                                                                                                                                                                                                                         &                   United Nations Development Programme: Human Development Reports \cite{UN}                                                                                                                                                                                  \\ \midrule
Latitud                              & LAT    & Static     &  &    United Nations Development Programme: Human Development Reports \cite{UN}                                                                                                                                                                                                                                                                                                       &                                           \\ \midrule
Longitude                           & LON    & Static  &     &   United Nations Development Programme: Human Development Reports \cite{UN}                                                                                                                                                                                                                                                                             &                                                                                                                                                                                            \\ \midrule
Altitude                            & AL     & 2018         & Average altitude in the affected area. Units: m                                                    & SRTM Digital Elevation Data Version 4. 90m Resolution.  http://srtm.csi.cgiar.org/     \\ \midrule                                                                                                                                                                   
Arable Land & ARL    & 2018         & Percentage of land cultivated for crops like wheat, maize, and rice that are replanted after each harvest in a country.                                                                                                                                                                  &  United Nations Development Programme: Human Development Reports \cite{UN}                                                                                                                                                                                                                                                                                                         \\ \midrule
Enhanced Vegetation Index & EVI  & 2017-2019 & EVI is an enhanced vegetation index designed to improve vegetation signal in regions with high biomass by reducing atmospheric effects. Used criteria for the value is low clouds, low vision angle and the highest value of EVI. & MOD13A2.006 Terra Vegetation Indices 16-Day Global 1km.
\cite{modis} \\
\midrule
\multicolumn{5}{l}{{\bf Domain: \textit{Political Index}}}\\ 
\midrule
Corruption Index                      & COR    & 2018         &        Captures the degree of perception of which public charges use public capital for private interests                                                                                                                                                                                          &                      Worldwide Governance Indicators \cite{WFI}                                                                                                                                                                                                                                                                                   \\ \midrule
Goverment Effectiveness                        & GE     & 2018         &    Captures the perceptions on the quality of public services, civil services and their independence from political pressures as well as the perception on credibility, compromise and quality of govermental policies.                                                                                                                                                                                                                                                                                                                                                                                 &          Worldwide Governance Indicators \cite{WFI}                                                                                                                                                                                                                                                                                               \\ \midrule
Absence of Violence                                   & AV     & 2018         &   Measures the perception and cases on political instability and absence of violence and terrorism.                                                                                                                                                                                               &          Worldwide Governance Indicators \cite{WFI}                                                                                                                                                                                                                                                                                               \\ \midrule
Regulatory Quality                    & RQ     & 2018         &      Captures the perception of the ability of a goverment to enforce effective policies and regulations.                                                                                              &           Worldwide Governance Indicators \cite{WFI}                                                                                                                                                                              \\ \midrule
Rule of Law                           & RL     & 2018         & Captures perception on the quality of laws and the degree of fairness in which the law is applied   &                Worldwide Governance Indicators \cite{WFI}                                                                                                                 \\ \midrule
Voice Accountability                  & VA     & 2018         &   Captures the perceptions on the level in which citizens from a country can actively engage with the selection of its goverment, freedom of speech, association and media.  &                                   Worldwide Governance Indicators \cite{WFI}                                                                                                                                                   \\ \bottomrule \bottomrule

\end{tabular}
\end{footnotesize}
